Supervised Learning via Ensembles of Diverse Functional Representations: the Functional Voting Classifier

Many conventional statistical and machine learning methods face challenges when applied directly to high dimensional temporal observations. In recent decades, Functional Data Analysis (FDA) has gained widespread popularity as a framework for modeling and analyzing data that are, by their nature, functions in the domain of time. Although supervised classification has been extensively explored in recent decades within the FDA literature, ensemble learning of functional classifiers has only recently emerged as a topic of significant interest. Thus, the latter subject presents unexplored facets and challenges from various statistical perspectives. The focal point of this paper lies in the realm of ensemble learning for functional data and aims to show how different functional data representations can be used to train ensemble members and how base model predictions can be combined through majority voting. The so-called Functional Voting Classifier (FVC) is proposed to demonstrate how different functional representations leading to augmented diversity can increase predictive accuracy. Many real-world datasets from several domains are used to display that the FVC can significantly enhance performance compared to individual models. The framework presented provides a foundation for voting ensembles with functional data and can stimulate a highly encouraging line of research in the FDA context.

==> application.tex <==
if hard voting:
    binarize all the outcome variables (set all values != 1 to 0)
For each dataset:

1) RUN EXPERIMENTS

    for basis in [ 'B-spline3', 'B-spline5', 'Fourier']: 
        for n between 7 and K*
            train KNN, RF, GB, DT with 10-fold CV

*K = min(time instances, 500)
*only multiples of 3

2) Save results in results.csv

3) Group by ['Model', 'dataset', 'basis'] and select the max value for the CV accuracy on the test set.

4) Save in resultsbest.csv. In this table we have the best models, 3 on each (dataset, basis) combination

5) Voting ensemble
for model in [KNN, RF, DT, GB]:
    if soft voting:
        get predicted probabilities for each class**  
    elif hard voting:
        get predicted classes

if hard voting:
    output the ensemble prediction as the majority vote
    select the class with the highest probability as output.

elif soft voting:
    average the probabilities


**how the different models output probabilities:
KNN
In the k-nearest neighbors algorithm with k=5, if a new data point has three neighbors of class A and two of class B, the algorithm would predict the data point as class A, with probabilities [0.6, 0.4], based on the ratio of the classes in the nearest neighbors.

RF
The predicted class probabilities of an input sample are computed as the mean predicted class probabilities of the trees in the forest. The class probability of a single tree is the fraction of samples of the same class in a leaf.

DT
The predicted class probability is the fraction of samples of the same class in a leaf.
 
